A Review of Reinforcement Learning in Financial Applications

In recent years, there has been a growing trend of applying Reinforcement Learning (RL) in financial applications. This approach has shown great potential to solve decision-making tasks in finance. In this survey, we present a comprehensive study of the applications of RL in finance and conduct a series of meta-analyses to investigate the common themes in the literature, such as the factors that most significantly affect RL's performance compared to traditional methods. Moreover, we identify challenges including explainability, Markov Decision Process (MDP) modeling, and robustness that hinder the broader utilization of RL in the financial industry and discuss recent advancements in overcoming these challenges. Finally, we propose future research directions, such as benchmarking, contextual RL, multi-agent RL, and model-based RL to address these challenges and to further enhance the implementation of RL in finance.

==> Tables/old_tables.tex <==
\begin{table}
\begin{tabular}{ | m{2cm} | m{2.5cm}| m{2.5cm} | m{2.5cm} |m{1.7cm} |m{2cm} | m{2cm} | } 
% \begin{tabular}{ | | |  |  || | } 
  \hline
  Study & State & Action & Reward & Algorithm & Data & Contribution\\ 
  \hline

\citet{ chan2001electronic} & inventory of agent, order imbalance, bid-ask spread and some other market quantity measures functions of price change, etc.)& change in bid and ask prices & a linear combination of profit, inventory risk and
market quality & SARSA and actor-critic algorithm with policy by Boltzmann distribution & Using the simulator of their own & The first to apply RL in market making
\\
\hline


  \citet{Patel2018MM} & Macro agent: historical price data; Market Indicator Features (Price Level, Price Change, Volume Level,
Volume Change, Volatility); Micro agent: time, inventory, end-to-end market information & Macro agent: Buy, sell, or hold the asset; Micro agent: price of limit orders & Macro agent: clipped reward of profit based on decision; Micro agent: profit based on price difference & DQN & Bitcoin data based on historical orderbook& Propose a novel hierarchical decision structure for Market Making Agent\\ 
  \hline
  
  % \citet{Patel2018MM} & Macro agent: historical price data; Market Indicator Features (Price Level, Price Change, Volume Level,Volume Change, Volatility) & Macro agent: Buy, sell, or hold  & Macro agent: clippted reward based on decisionprice information, inventory information, volatility; micro agent: bid-ask information, trade information & Macro agent: Buy, sell, or hold ; micro agent: price of limit order & Macro agent: clippted reward based on decision;  micro agent:  a function of Volume Weighted Average Price& DQN & Bitcoin data based on historical orderbook& Propose a novel hierarchical decision structure for Mmarket Mmaking Aagent\\ 
  % \hline

  
  \citet{Spooner2018MM} & Inventory, active quoting distances, and 
market states (market spread, mid-price move,
book/queue imbalance, signed volume, 
volatility, relative strength index) & Place limit orders at fixed distances to the mid-price; Clear inventory  &  PnL from placing orders and inventory PnL, with asymmetrically dampened reward function designed to encourage making orders rather than profiting from speculation (keeping the inventory) & Q-learning, 
SARSA 
and R-learning & Data from their simulator, which is developed based on historical data & Propose the asymmetrically dampened reward function\\
%   \hline
%   \citet{spooner2020robust} & Current time and the agent's inventory &   Quoted spread and reservation price & Mark-to-market
% (MtM) value of the agent's holding (include both profit of executing orders and value change of the holding) &  NAC-S($\lambda$) algorithm & Data generated by a simulator & Proposes adversarial RL in market making\\
%   \hline
%   \citet{gavsperov2021market} &  Agent’s inventory; price range and trend predictions  & placing bid/ask orders with distances in tick size
% relative to the current best bid/ask  & symmetrically dampened PnL reward function in \cite{Spooner2018MM}, and inventory penalizing term & Policy gradient with fully-connected neural network & Bitstamp
% for the pair Bitcoin/US Dollar
% \\
  \hline
  
  \citet{Ganesh2019MM} & Trades executed in previous time step; Inventory; Reference 
mid-price and spread curves; Market share; & Pricing; Hedging;  & Total PnL with different penalty for inventory PnL & PPO & Data generated by their own simulator & Introduce a competing MM agent and let RL agent to learn its behavior\\ 
  \hline
\end{tabular}




\caption{RL Methods in Market Making}
\label{table:market_making}
\end{table}

\begin{table}[]
    \label{table:market_making_2}
    \caption{RL Methods in Market Making}
    \centering
\begin{tabular}{| m{2cm} | m{2.5cm}| m{2.5cm} | m{2.5cm} |m{1.7cm} |m{2cm} | m{2cm} |} 
  \hline
  Study & State & Action & Reward & Algorithm & Data & Contribution\\
  \hline
  \citet{mani2019applications} & volume imbalance and the market-maker’s bid-ask spread &changes in the
market-maker’s ask and bid quotes &a linear function of profit, inventory penalty 
and market-maker’s bid-ask spread & SARSA and Double SARSA & Using the simulator of their own & Use risk sensitive RL in market making
\\
  \hline
  \citet{spooner2020robust} & Current time and the agent's inventory &   Quoted spread and reservation price & Mark-to-market
(MtM) value of the agent's holding with penalty term of terminal inventory &  NAC-S($\lambda$) algorithm & Data generated by a simulator & Proposes adversarial RL in market making\\
  \hline
  \citet{gavsperov2021market} &  Agent’s inventory; price range and trend predictions  & placing bid/ask orders with distances in tick size
relative to the current best bid/ask  & symmetrically dampened PnL reward function in \cite{Spooner2018MM}, and inventory penalizing term & Policy optimization by genetic algorithms & Bitstamp
for the pair Bitcoin/US Dollar& Use  signal generating unit to predict price change
\\
\hline

\citet{selser2021optimal} & mid-price of the asset, inventory of the agent,  and time & (discretized) bid price and ask price &a profit minus the estimated variance of profit with a constant & Deep Q-Learning and Tabular Q-Learning & Using the simulator of their own & Use a mean minus variance formulation of reward to recover the optimal agent  
\\
\hline

\citet{haider2021gaussian} & volatility, relative strength index,
book imbalance, inventory, ask level and bid level & Place limit
orders at
fixed distances
to the mid-
price; Clear
inventory & a variant of asymmetrically dampened reward function proposed in \citet{Spooner2018MM} & Gaussian distribution based nonlinear
function approximation (GBNLFA, a variant of SARSA) & Data from their simulator, which is developed based on historical data & Propose the RL algorithm GBNLFA to handle function approximation from continuous states to discrete actions
\\
\hline


\end{tabular}
\end{table}


\begin{table}[H]
\caption{Surveyed paper for Reinforcement Learning in Portfolio Management}
\label{table:multi_stage_portfolio_management}
\begin{tabular}{| m{2cm} | m{3cm}| m{2.5cm} | m{2.5cm} |m{1.7cm} |m{2.3cm} | }
\hline
Application & State& Action & Reward & Algorithm& Data \\ \hline
\cite{jiang2017deep} & Prices, Portfolio& Asset Allocation Weight & Return& Policy Gradient& Cryptocurrency \\ \hline
\cite{yu2019model}& Prices, Portfolio, Market Indicators, Predictions & Asset Allocation Weight & Return& DDPG& Stock \\ \hline
\cite{zhang2020deep} & Prices, Portfolio, Technical Indicators& Long/Hold/Short & Volatility-Adjusted Return & PG, DQN, A2C & Futures \\ \hline
\cite{ye2020reinforcement} & Prices, Predictions & Asset Allocation Weight & Return& Policy Gradient& Cryptocurrency, Stock \\ \hline
\cite{nan2020sentiment} & Prices, Portfolio, Predictions & Long/Hold/Short & Return& DQN & Stock \\ \hline
\cite{wang2021deeptrader} & Prices, Market Indicators, Predictions & Asset Allocation Weight & Return& Policy Gradient& Stock \\ \hline
\cite{wang2021commission} & Prices, Portfolio, LOB, Predictions & Asset Allocation Weight, Long/Hold/Short & Return& Reinforce, Double-Q & Stock \\ \hline
\cite{benhamou2020aamdrl} & Prices, Market Indicators & Asset Allocation Weight & Return& Policy Gradient& Portfolio, Strategies \\ \hline
\cite{benhamou2021detecting} & Prices, Portfolio, Market Indicators & Asset Allocation Weight & Return& Policy Gradient& Portfolio, Strategies \\ \hline
\end{tabular}
\end{table}


\input{Tables/table_optimal_execution}


==> Tables/table_market_making.tex <==


\begin{table}[]
\caption{Literature on RL methods in market making: state and actions.
}
\label{newtable:market_making_2}
\begin{tabular}{c|c|ccccccccc|cccc}
\cline{1-15} 
\multirow{2}{*}{Study}             & \multirow{2}{*}{Application}                                     & \multicolumn{9}{c|}{State}                                                                                                                                                                                                                                            & \multicolumn{2}{c}{Action}                                                                                            \\ \cline{3-15} 
                                   &                                                       & \rotatebox{90}{Price} & \rotatebox{90}{Inventory/Portfolio} & \rotatebox{90}{Market Indicator} & \rotatebox{90}{Technical Indicator} & \rotatebox{90}{Predictions} & \rotatebox{90}{Bid-ask information} & \rotatebox{90}{Trading Volume} & \rotatebox{90}{E2E} & \rotatebox{90}{Time} & \rotatebox{90}{Place limit order} & \rotatebox{90}{Clear Inventory} \\ \hline
% \multirow{9}{*}{\rotatebox{90}{MM}}

& \cite{chan2001electronic}    & \cmark                & \cmark                              &                                  &                                     &                             & \cmark                       &                      &                         &                      & \cmark                            &                            &                           &                          \\

& \cite{Patel2018MM}    & \cmark                & \cmark                             &                                  &                                     &                             &                        &  \cmark                       &  \cmark                       & \cmark                     & \cmark                            &                            &                           &                          \\


& \cite{Spooner2018MM}    & \cmark                & \cmark                              &                                  &   \cmark                                   &                             &  \cmark                        &     \cmark                    &                         &                      & \cmark                            & \cmark                            &                           &                          \\

& \cite{Ganesh2019MM}    & \cmark                & \cmark                              &                                  &                                    &                             &  \cmark                        &     \cmark                    &                         &                      & \cmark                            &                            &                           &                          \\

& \cite{mani2019applications}    &              &                            &                                  &                                    &                             &  \cmark                        &                        &                         &                      & \cmark                            &                            &                           &                          \\

& \cite{spooner2020robust}    &              &  \cmark                          &                                  &                                    &                             &                      &                      &                         &   \cmark                   & \cmark                            &                            &                           &                          \\

& \cite{gavsperov2021market}    &   \cmark              &  \cmark                          &                                  &                                    &    \cmark                            &                      &                      &                         &                 & \cmark                            &                            &                           &                          \\

& \cite{selser2021optimal}    &   \cmark              &  \cmark                          &                                  &                                    &                                &                      &                      &                         &   \cmark              & \cmark                            &                            &                           &                          \\

& \cite{haider2021gaussian}    & \cmark                &  \cmark                          &                                  &     \cmark                                 &                                &   \cmark                      &                        &                         &                 & \cmark                            &  \cmark                           &                           &                          \\

          \cline{1-15} 
\end{tabular}
\end{table}


 \begin{table}[]
\caption{Literature on RL methods in Market Making: reward and algorithm. 
}
\label{table:TODO}
\begin{tabular}{c|c|ccccccc|cccccc}
\cline{1-15} 
\multirow{2}{*}{Application} & \multirow{2}{*}{Paper} & \multicolumn{9}{c|}{Reward} & \multicolumn{4}{c}{Algorithm} \\ \cline{3-15} 
 & & \rotatebox{90}{PnL} & \rotatebox{90}{Return} & \rotatebox{90}{VR} & \rotatebox{90}{IS} & \rotatebox{90}{Shaped reward} & \rotatebox{90}{Inventory Penalty} & \rotatebox{90}{Market Quality} & \rotatebox{90}{Critic-only} & \rotatebox{90}{Actor-only} & \rotatebox{90}{Actor-critic} \\ \hline
\multirow{9}{*}{\rotatebox{90}{Market Making}} 
& \cite{chan2001electronic} &\cmark &  & & & &\cmark &\cmark      &\cmark & & \cmark \\
& \cite{Patel2018MM} &\cmark &  & & & & &          &\cmark & &  \\
& \cite{Spooner2018MM} &\cmark &  & & & &\cmark &          &\cmark & &  \\
& \cite{Ganesh2019MM} &\cmark &  & & & &\cmark &          & &\cmark &  \\
& \cite{mani2019applications} &\cmark &  & & & &\cmark & \cmark         &\cmark & &  \\
& \cite{spooner2020robust} &\cmark &  & & & &\cmark &         & &\cmark &  \\
& \cite{gavsperov2021market} &\cmark &  & & & &\cmark &         & &\cmark &  \\
& \cite{selser2021optimal} &\cmark &  & & & & &         &\cmark & &  \\
& \cite{haider2021gaussian} &\cmark &  & & & &\cmark  &         &\cmark & &  \\

\cline{1-15} 

\end{tabular}
\end{table}

==> Tables/table_multi_stage_portfolio_management.tex <==
% \begin{table}[]
% %\resizebox{\textwidth}{!}{%
% \begin{tabular}{@{}lllll@{}}
% \hline
% Paper & MDP & Algorithm & Data & Contribution \\
% \hline
%\citet{jiang2017deep} & 
%\begin{tabular}[c]{@{}l@{}}State: Stock price and asset weight at prior time\\ Action:\\ Reward\end{tabular} & 
%\acrshort{DPG}& 
%11 top volume cryptocurrencies & 
%Proposed "Ensemble of Identical Independent Evaluators""; Applied a stochastic mini-batch online learning scheme\\
% \hline
%\citet{ye2020reinforcement} & \begin{tabular}[c]{@{}l@{}}State\\ Action\\ Reward\end{tabular} & & & \\
% \hline
%\citet{nan2020sentiment} & & & & \\
% \hline
%\citet{liang2018adversarial} & & & & \\
% \hline
%\citet{liu2020adaptive} & & & & \\
% \hline
%\citet{zhang2020deep} & & & & \\
% \hline
%\citet{wang2021commission} & & & & \\
% \hline 
%\citet{wang2021deeptrader} & & & & \\
% \hline
% \end{tabular}
% %%
% %}
% \label{table:multi_stage_portfolio_management}
% \caption{PM}
% \end{table}


% \begin{table}[H]
% \begin{tabular}{| m{2cm} | m{2.5cm}| m{2.5cm} | m{2cm} |m{1.7cm} |m{2.5cm} | m{2cm} |}
% \hline
% Application & State & Action & Reward & Algorithm& Data & Contribution \\ \hline
% \cite{jiang2017deep} & Asset Info Portfolio Info & Asset Allocation Weight & Return& Policy Gradient& Cryptocurrency & \\ \hline
% \cite{yu2019model}& Asset Info Portfolio Info, Market Indicators, Other & Asset Allocation Weight & Return& DDPG& Stock & \\ \hline
% \cite{zhang2020deep} & Asset Info Portfolio Info, Technical Indicators& Long/Short Proportion & Volatility-Adjusted Return & PG, DQN, A2C & Futures & \\ \hline
% \cite{ye2020reinforcement} & Asset Info Other & Asset Allocation Weight & Return& Policy Gradient& Cryptocurrency, Stock & \\ \hline
% \cite{nan2020sentiment} & Asset Info, Portfolio Info, Other & Long/Hold/Short Proportion & Return& DQN & Stock & \\ \hline
% \cite{wang2021deeptrader} & Asset Info, Market Indicators, Other& Asset Allocation Weight & Return& Policy Gradient& Stock & \\ \hline
% \cite{wang2021commission} & Asset Info, Portfolio Info, LOB, Other & Asset Allocation Weight, Long/Hold/Short & Return& Reinforce, Double-Q & Stock & \\ \hline
% \cite{benhamou2020aamdrl} & Asset Info Market Indicators & Asset Allocation Weight & Return& Policy Gradient& Portfolio/Strategies & \\ \hline
% \cite{benhamou2021detecting} & Asset InfoPortfolio Info, Market Indicators & Asset Allocation Weight & Return& Policy Gradient& Portfolio/Strategies & \\ \hline
% \end{tabular}
% \label{table:multi_stage_portfolio_management}
% \caption{Surveyed paper for Reinforcement Learning in Portfolio Management}
% \end{table}


% \begin{table}[]
% % \begin{tabular}{mmmmmm}
% \begin{tabular}{| m{2cm} | m{2.5cm}| m{2.5cm} | m{2.5cm} |m{1.7cm} |m{2cm} | }
% \hline
% Application & State & Action & Reward & Algorithm & Data \\ \hline
% A deep reinforcement learning framework for the financial portfolio management problem & Price (low, high, close) normalized by the latest closing price; Internal state is the weight at t-1. & Weights vector to determine portfolio allocation. & Final portfolio value, i.e. average logarithmic cumulated return. & DPG& Top 11 volume bitcoin trading information from Poloniex \\ \hline
% Reinforcement-Learning-based Portfolio Management with Augmented Asset Movement Prediction States & Price (low, high, close); Articles from the news. & Weights vector to determine portfolio allocation. & Final portfolio value, i.e. average logarithmic cumulated return. & DPG; PPO; PG & Bitcoin data; stock from HighTech companies\\ \hline
% Adversarial Deep Reinforcement Learning in Portfolio Management & Price (low, high, close); Volume; Other financial indexes.& Weights vector to determine portfolio allocation. & Cumulative return subtract portfolio volatility & DDPG; PPO; PG& Use data from a simulator which is developed based on historical data \\ \hline
% %%
% Model-based deep reinforcement learning for dynamic portfolio optimization & Price (low, high, close); Augmented states (predicted future price change percentage) & Weights vector to determine portfolio allocation. & Final portfolio value, i.e. average logarithmic cumulated return. & DDPG & Company stocks\\ \hline
% %%
% Adaptive Quantitative Trading An Imitative Deep Reinforcement Learning Approach & Account observation set, Market observation set& Long or short & Sharpe ratio differential & Imitative Recurrent DPG & CHINA IC, IF \\ \hline
% %%
% \end{tabular}
% \caption{PM}
% \end{table}

% \multirow{9}{*}{\rotatebox{0}{\makecell{Portfolio \\ Management}}}

% \begin{table}[]
% \begin{tabular}{l|l|lllllllll|llll}
% \multirow{2}{*}{Application} & \multirow{2}{*}{Paper} & \multicolumn{9}{l|}{State} & \multicolumn{4}{l}{Action} \\ \cline{3-15} 
% & & \rotatebox{90}{Price} & \rotatebox{90}{Inventory/Portfolio} & \rotatebox{90}{Market Indicator} & \rotatebox{90}{Technical Indicator} & \rotatebox{90}{Predictions} & \rotatebox{90}{Spread} & \rotatebox{90}{Volume} & \rotatebox{90}{E2E/LOB} & \rotatebox{90}{Time} & \rotatebox{90}{Allocation Weight} & \rotatebox{90}{Long/Short} & \rotatebox{90}{Bid Price} & \rotatebox{90}{Quantity} \\ \hline
% \cite{jiang2017deep} & \multirow{9}{*}{\rotatebox{90}{Portfolio Management}} & \cmark& \cmark & & & & & & & & \cmark & & & \\
% \cite{yu2019model} & & \cmark& \cmark & \cmark& & \cmark& & & & & \cmark & & & \\
% \cite{zhang2020deep} & & \cmark& \cmark & & \cmark & & & & & & & \cmark & & \\
% \cite{ye2020reinforcement} & & \cmark& & & & & & & & & \cmark & & & \\
% \cite{nan2020sentiment} & & \cmark& \cmark & & & & & & & & & \cmark & & \\
% \cite{wang2021deeptrader}& & \cmark& & \cmark& & \cmark& & & & & \cmark & & & \\
% \cite{wang2021commission}& & \cmark& \cmark & & & \cmark& & & \cmark & & \cmark & & & \\
% \cite{benhamou2020aamdrl}& & \cmark& & \cmark& & & & & & & \cmark & & & \\
% \cite{benhamou2021detecting} & & \cmark& \cmark & \cmark& & & & & & & \cmark & & & \\ \cline{2-15} 
% \citet{nevmyvaka2006reinforcement} & 
% \multirow{8}{*}{\rotatebox{90}{Optimal Execution}} & & \cmark & & & & \cmark & \cmark & & \cmark & & & \cmark & \\
% \citet{deng2016deep} & & \cmark& & & & & & & & & & \cmark & & \\
% \citet{wei2019model} & & & \cmark & & & & & & \cmark & & & & & \cmark \\
% \citet{lin2020E2E} & & & \cmark & & & & & & \cmark & & & & & \cmark \\
% \citet{fang2021universal}& & \cmark& \cmark & & & & & \cmark & & \cmark & & & & \cmark \\
% \citet{lin2020deep}& & \cmark& \cmark & & & & \cmark & & \cmark & & & & & \cmark \\
% \citet{shen2014risk} & & & \cmark & & & & \cmark & & & & & & \cmark & \\
% \citet{hendricks2014reinforcement} & & & \cmark & & & & \cmark & \cmark & & \cmark & & & & \cmark 
% \end{tabular}
% \end{table}


% Portfolio
% E2E

\begin{table}[]
\caption{Literature on RL methods: state and actions. 
}
\label{table:TODO}
\begin{tabular}{c|c|ccccccccc|cccc}
\cline{1-15} 
\multirow{2}{*}{Application} & \multirow{2}{*}{Paper} & \multicolumn{9}{c|}{State} & \multicolumn{4}{c}{Action} \\ \cline{3-15} 
 & & \rotatebox{90}{Price} & \rotatebox{90}{Inventory} & \rotatebox{90}{Market Indicator} & \rotatebox{90}{Technical Indicator} & \rotatebox{90}{Predictions} & \rotatebox{90}{Bid-ask information} & \rotatebox{90}{Trading Volume} & \rotatebox{90}{E2E} & \rotatebox{90}{Time} & \rotatebox{90}{Allocation Weight} & \rotatebox{90}{Long/Short} & \rotatebox{90}{Bid Price} & \rotatebox{90}{Quantity} \\ \hline
\multirow{9}{*}{\rotatebox{90}{Portfolio Management}} & \cite{jiang2017deep} & \cmark& \cmark & & & & & & & & \cmark & & & \\
 & \cite{yu2019model} & \cmark& \cmark & \cmark& & \cmark& & & & & \cmark & & & \\
 & \cite{zhang2020deep} & \cmark& \cmark & & \cmark & & & & & & & \cmark & & \\
 &\cite{ye2020reinforcement} & \cmark& & & & & & & & & \cmark & & & \\
 &\cite{nan2020sentiment}& \cmark& \cmark & & & & & & & & & \cmark & & \\
 &\cite{wang2021deeptrader} & \cmark& & \cmark& & \cmark& & & & & \cmark & & & \\
 & \cite{wang2021commission} & \cmark& \cmark & & & \cmark& & & \cmark & & \cmark & & & \\
 & \cite{benhamou2020aamdrl} & \cmark& & \cmark& & & & & & & \cmark & & & \\
& \cite{benhamou2021detecting} & \cmark& \cmark & \cmark& & & & & & & \cmark & & & \\ \cline{1-15} 
\multirow{8}{*}{\rotatebox{90}{Optimal Execution}} & 
\citet{nevmyvaka2006reinforcement} & & \cmark & & & & \cmark & \cmark & & \cmark & & & \cmark & \\
 & \citet{deng2016deep} & \cmark& & & & & & & & & & \cmark & & \\
 & \citet{wei2019model} & & \cmark & & & & & & \cmark & & & & & \cmark \\
 & \citet{lin2020E2E} & & \cmark & & & & & & \cmark & & & & & \cmark \\
 & \citet{fang2021universal} & \cmark& \cmark & & & & & \cmark & & \cmark & & & & \cmark \\
& \citet{lin2020deep} & \cmark& \cmark & & & & \cmark & & \cmark & & & & & \cmark \\
 & \citet{shen2014risk} & & \cmark & & & & \cmark & & & & & & \cmark & \\
 &\citet{hendricks2014reinforcement} & & \cmark & & & & \cmark & \cmark & & \cmark & & & & \cmark \\\cline{1-15} 
\end{tabular}
\end{table}



 \begin{table}[]
\caption{Literature on RL methods: reward and algorithm. 
}
\label{table:TODO}
\begin{tabular}{c|c|ccccccc|cccccc}
\cline{1-15} 
\multirow{2}{*}{Application} & \multirow{2}{*}{Paper} & \multicolumn{9}{c|}{Reward} & \multicolumn{4}{c}{Algorithm} \\ \cline{3-15} 
 & & \rotatebox{90}{PnL} & \rotatebox{90}{Return} & \rotatebox{90}{VR} & \rotatebox{90}{IS} & \rotatebox{90}{Shaped reward} & \rotatebox{90}{Inventory Penalty} & \rotatebox{90}{Market Quality} & \rotatebox{90}{DQN} & \rotatebox{90}{PG} & \rotatebox{90}{PPO} & \rotatebox{90}{simulator} & \rotatebox{90}{TBD} & \rotatebox{90}{TBD} \\ \hline
\multirow{9}{*}{\rotatebox{90}{Portfolio Management}} 
& \cite{jiang2017deep} & & \cmark & & & & & & & & & \red{TBD} & & \\
 & \cite{yu2019model} & & \cmark & & & & & & & & & & & \\
 & \cite{zhang2020deep} & & \cmark & & & & & & & & & & & \\
 &\cite{ye2020reinforcement} & & & \cmark & & & & & & & & & & \\
 &\cite{nan2020sentiment} & & \cmark & & & & & & & & & & & \\
 &\cite{wang2021deeptrader} & & \cmark & & & & & & & & & & & \\
 & \cite{wang2021commission} & & \cmark & & & & & & & & & & & \\
 & \cite{benhamou2020aamdrl} & & \cmark & & & & & & & & & & & \\
& \cite{benhamou2021detecting} & & \cmark & & & & & & & & & & & \\ \cline{1-15} 
\multirow{8}{*}{\rotatebox{90}{Optimal Execution}} & 
\citet{nevmyvaka2006reinforcement} & \cmark & & & & & & & \cmark & & & & & \\
 & \citet{deng2016deep} & \cmark & & \cmark & & & & & & \cmark & & & & \\
 & \citet{wei2019model} &\cmark & & & & & & & & & & \cmark & & \\
 & \citet{lin2020E2E} & & & & \cmark & & & & & & \cmark & & & \\
 & \citet{fang2021universal} & & & & &\cmark & & & & & \cmark & & & \\
& \citet{lin2020deep} & & & & &\cmark & & & \cmark & & & & & \\
 & \citet{shen2014risk} & \cmark & & & & & & & \cmark & & & & & \\
 &\citet{hendricks2014reinforcement} & & & &\cmark & & & & \cmark & & & & & 
 \\\cline{1-15} 
\end{tabular}
\end{table}

==> Tables/table_optimal_execution.tex <==

% We introduce the following abbrevations. 
% For state, we use PA to denote Past Actions, Pos to denote the current Positions, xx. 
% For action, we use Qty to denote the quantity that we are going to place, Dir to denote the direction of this placement (negative or positive), and P to denote the price. 
% We use to emphasize it is discritized 

\begin{table}[t]
\caption{Literature on RL methods for Optimal Execution. 
}
\label{table:optimal_execution}
% 		\centering
% \hspace{-2cm}
% \small
% \renewcommand{\arraystretch}{1.5}
\begin{tabular}{m{2cm} llll}
    \hline
     Study & State & Action & Reward & Algorithm \\ %  & Data
\hline
%
   \citet{nevmyvaka2006reinforcement} & Inventory, Spread,  Time,  Volume
  &  bid price  &  PnL &  DQN \\ 
\hline
%
   \citet{deng2016deep} & Price  &  long/hold/short
  &\makecell{PnL \& VR}    & PG   \\ 
\hline
%
   \citet{wei2019model} & Inventory,  E2E
  &  quantity  & PnL  & \makecell{Simulator \\ \& model-free}   \\ 
\hline
%
   \citet{lin2020E2E} & Inventory,  Time,  E2E
  &  quantity  & IS  & PPO   \\ 
\hline
%
   \citet{fang2021universal} &  Inventory,  Price,  Time,   Volume
 &  quantity  & shaped reward  & PPO  \\ 
\hline
%
   \citet{lin2020deep} & Inventory,  Price,  Spread,  Time,  E2E
  &  quantity  & shaped reward  &  DQN  \\ 
\hline
%
   \citet{shen2014risk} &  Inventory,  Spread 
 &  bid price
  & PnL  &  DQN \\ 
\hline
%
   \citet{hendricks2014reinforcement} & Inventory,  Spread,   Time,  Volume  & quantity  &  IS & DQN  \\ 
  \hline
\end{tabular}
\end{table}











% \begin{table}

% \begin{tabular}{ | m{2cm}  m{2.5cm} m{2.5cm}  m{2.5cm} m{1.7cm} m{2cm} | } 
%   \hline
%   Reference & State & Action & Reward & Algorithm & Data/Simulator \\ 
%   \hline
%   %
%    \citet{nevmyvaka2006reinforcement} &   &    &   &   & \\ 
%   \hline
%   %
%    \citet{deng2016deep} &   &    &   &   & \\ 
%   \hline
%   %
%   \citet{wei2019model} &   & Qty, Dir    &  delta of middle price $\times$  Qty & DDQN/PG/A2C & \\ 
%   \hline
%   %
%   \citet{roa2019towards} &   &    &   & existing IRL methods & \\ 
%   \hline
%   %
%   \citet{karpe2020multi} &   &  Qty, P (d)  & price slippage $\times$  Qty & DDQN & \\ 
%   \hline
%   %
%    \citet{fang2021universal}  &   &    &   &   & \\ 
%   \hline
% \end{tabular}
% % \end{table}




% "private states = (time remaining, quantity remaining)
% market state variables = (bid-ask spread, volume imbalance, one-period price return, t-period price return)"


% past actions + current positions + AutoEncoder(past observations)

==> acronym.tex <==
\newacronym{LSTM}{LSTM}{Long Short Term Memory}
\newacronym{MDD}{MDD}{Maximum Drawdown}
\newacronym{fAPV}{fAPV}{Final Accumulative Portfolio Value}
\newacronym{SR}{SR}{Sharpe Ratio}
\newacronym{PAMR}{PAMR}{Passive Aggressive Mean Reversion}
\newacronym{ONS}{ONS}{ Online Newton Step}
\newacronym{PG}{PG}{Policy Gradient}
\newacronym{DPG}{DPG}{Deterministic Policy Gradient}
\newacronym{DDPG}{DDPG}{Deep Deterministic Policy Gradient}
\newacronym{DQN}{DQN}{Deep Q-learning Networks}
\newacronym{PPO}{PPO}{Proximal Policy Optimization}
\newacronym{TARO}{TARO}{Trust Region Policy Optimization}
\newacronym{A2C}{A2C}{Advantage Actor-Critic}
\newacronym{SARSA}{SARSA}{State–action–reward–state–action Algorithm}
\newacronym{RSI}{RSI}{Relative Strength Index}
\newacronym{MACD}{MACD}{Moving Average Convergence Divergence}
\newacronym{CNN}{CNN}{Convolutional Neural Network}
\newacronym{RNN}{RNN}{Recurrent Neural Network}

\newacronym{DRN}{DRN}{Deep Residual Network}
\newacronym{GAN}{GAN}{Generative Adversarial Network}
\newacronym{BCM}{BCM}{Behavior Cloning Module}
\newacronym{POMDP}{POMDP}{Partially Observable Markov Decision Process}
\newacronym{MDP}{MDP}{Markov Decision Process}
\newacronym{RDPG}{RDPG}{Recurrent Deterministic Policy Gradient}
\newacronym{DRL}{DRL}{Deep Reinforcement Learning}
\newacronym{RL}{RL}{Reinforcement Learning}
\newacronym{ML}{ML}{Machine Learning}
\newacronym{E2E}{E2E}{End-to-end information, including all Limit-order-book information}
\newacronym{LOB}{LOB}{Limit-order-book}
\newacronym{VR}{VR}{volatility-adjusted return}
\newacronym{PnL}{PnL}{Profit and Loss}
\newacronym{IS}{IS}{Implementation shortfall}
\newacronym{EIIE}{EIIE}{Ensemble of Identical Independent Evaluators}
\newacronym{HRPM}{HRPM}{Hierarchical Reinforced Portfolio Management}
\newacronym{OE}{OE}{Optimal Execution}
\newacronym{MBVE}{MBVE}{Model-Based Value Expansion}
\newacronym{MBMF}{MBMF}{Model-Based RL with Model-Free Fine-Tuning}
\newacronym{I2A}{I2A}{Imagination-Augmented Agents}
\newacronym{HER}{HER}{Hindsight Experience Replay}
\newacronym{C51}{C51}{Categorical 51-Atom DQN}
\newacronym{TD3}{TD3}{Twin Delayed DDPG}
\newacronym{DJIA}{DJIA}{Dow Jones Industrial Average}
\newacronym{MPT}{MPT}{Modern Portfolio Theory}
\newacronym{TS}{TS}{Thompson Sampling}


==> terminology.tex <==
The Relative Strength Index (RSI) is a technical analysis indicator that measures the magnitude of recent price changes to assess overbought or oversold conditions in a security or other asset. It is commonly used to identify potential reversal points in the price of an asset and to help traders make buy or sell decisions.

The RSI is calculated using the average of the gains and losses of an asset over a given period of time. Specifically, the RSI is calculated as the ratio of the average gain to the average loss over the specified time period, multiplied by 100. A high RSI value (above 70) indicates that an asset may be overbought, while a low RSI value (below 30) indicates that it may be oversold.

The RSI is often used in conjunction with other technical analysis indicators, such as moving averages, to provide a more comprehensive view of an asset's price trends and potential entry or exit points for trades. It is also widely used in algorithmic trading systems to help automate the decision-making process.


